Debiasing with Diffusion: Probabilistic reconstruction of Dark Matter fields from galaxies with CAMELS

Galaxies are biased tracers of the underlying cosmic web, which is dominated by dark matter components that cannot be directly observed. Galaxy formation simulations can be used to study the relationship between dark matter density fields and galaxy distributions. However, this relationship can be sensitive to assumptions in cosmology and astrophysical processes embedded in the galaxy formation models, that remain uncertain in many aspects. In this work, we develop a diffusion generative model to reconstruct dark matter fields from galaxies. The diffusion model is trained on the CAMELS simulation suite that contains thousands of state-of-the-art galaxy formation simulations with varying cosmological parameters and sub-grid astrophysics. We demonstrate that the diffusion model can predict the unbiased posterior distribution of the underlying dark matter fields from the given stellar mass fields, while being able to marginalize over uncertainties in cosmological and astrophysical models. Interestingly, the model generalizes to simulation volumes approximately 500 times larger than those it was trained on, and across different galaxy formation models. Code for reproducing these results can be found at https://github.com/victoriaono/variational-diffusion-cdm

==> conclusion.tex <==
\section{Conclusion}
We have presented a diffusion generative model that can sample the posterior distribution of dark matter density fields conditioned on observable stellar maps. Previous deep learning approaches used regression-based frameworks, but we show that a generative model can be used to turn this mapping into a probabilistic one and capture the inherent uncertainty of the model due to lacking information in the stellar maps. The diffusion model can generate DM density fields with summary statistics and visual inspections consistent to those in the authentic simulations.
